Output Controllability of a Linear Dynamical System with Sparse Controls

In this paper, we study the conditions to be satisfied by a discrete-time linear system to ensure output controllability using sparse control inputs. A set of necessary and sufficient conditions can be directly obtained by extending the Kalman rank test for output controllability. However, the verification of these conditions is computationally heavy due to their combinatorial nature. Therefore, we derive non-combinatorial conditions for output sparse controllability which can be verified with polynomial time complexity. Our results also provide bounds on the minimum sparsity level required to ensure output controllability of the system. This additional insight is useful for designing sparse control input that drives the system to any desired output.

==> Supporting_Files/My_notations.tex <==
\crefname{app}{Appendix}{Appendices}
\crefname{cor}{Corollary}{Corollaries}
\crefname{prop}{Proposition}{Propositions}
\crefname{lemma}{Lemma}{Lemmas}
\crefname{defn}{Definition}{Definitions}
\crefname{conj}{Conjecture}{Conjectures}
\crefname{exam}{Example}{Examples}


\newtheorem{theorem}{Theorem}
\newtheorem{cor}{Corollary}
\newtheorem{lemma}{Lemma}
\newtheorem{prop}{Proposition}
\newtheorem{conj}{Conjecture}
\newtheorem{defn}{Definition}
\newtheorem{exam}{Example}

\newcommand{\bs}{\boldsymbol}
\newcommand{\bb}{\mathbb}
\newcommand{\mcal}{\mathcal}

\newcommand{\eye}{\bs{I}}
\newcommand{\zero}{\bs{0}}
\newcommand{\one}{\bs{1}}

\newcommand{\lb}{\left(}
\newcommand{\rb}{\right)}
\newcommand{\ls}{\left[}
\newcommand{\rs}{\right]}
\newcommand{\lc}{\left\{}
\newcommand{\rc}{\right\}}
\newcommand{\ld}{\left.}
\newcommand{\rd}{\right.}
\newcommand{\lv}{\left\vert}
\newcommand{\rv}{\right\vert}
\newcommand{\lV}{\left\Vert}
\newcommand{\rV}{\right\Vert}
\newcommand{\lan}{\left\langle}
\newcommand{\ran}{\right\rangle}
\newcommand{\lcl}{\left\lceil}
\newcommand{\rcl}{\right\rceil}
\newcommand{\LRV}[1]{{\left\vert\kern-0.25ex\left\vert\kern-0.25ex\left\vert #1 \right\vert\kern-0.25ex\right\vert\kern-0.25ex\right\vert}}


\newcommand{\nat}{\bb{N}}
\newcommand{\expect}[2]{\bb{E}_{#1}\lc#2\rc}
\newcommand{\indi}[1]{\mathbbm{1}_{\lc#1\rc}}
\newcommand{\nth}{^\mathsf{th}}
\newcommand{\tran}{^{\mathsf{T}}}
\newcommand{\T}{\mathsf{T}}
\newcommand{\trace}[1]{\mathsf{Tr}\lc#1\rc}
\newcommand{\diag}[1]{\mathsf{Diag}\lc#1\rc}
\newcommand{\rank}[1]{\mathsf{Rank}\lc#1\rc}
\newcommand{\DIA}[1]{\mathcal{D}\lc#1\rc}
\newcommand{\supp}[1]{\mathsf{Supp}\lc#1\rc}
\newcommand{\Vect}[1]{\mathsf{vec}\lc#1\rc}
\newcommand{\range}[1]{\mathcal{CS}\lc#1\rc}

\newcommand{\Gauss}{\mathcal{N}}

\newcommand{\matA}{\bs{A}}
\newcommand{\matB}{\bs{B}}
\newcommand{\matC}{\bs{C}}
\newcommand{\matD}{\bs{D}}
\newcommand{\matE}{\bs{E}}
\newcommand{\matF}{\bs{F}}
\newcommand{\matG}{\bs{G}}
\newcommand{\matH}{\bs{H}}
\newcommand{\matI}{\bs{I}}
\newcommand{\matJ}{\bs{J}}
\newcommand{\matK}{\bs{K}}
\newcommand{\matL}{\bs{L}}
\newcommand{\matM}{\bs{M}}
\newcommand{\matN}{\bs{N}}
\newcommand{\matO}{\bs{O}}
\newcommand{\matP}{\bs{P}}
\newcommand{\matQ}{\bs{Q}}
\newcommand{\matR}{\bs{R}}
\newcommand{\matS}{\bs{S}}
\newcommand{\matT}{\bs{T}}
\newcommand{\matU}{\bs{U}}
\newcommand{\matV}{\bs{V}}
\newcommand{\matW}{\bs{W}}
\newcommand{\matX}{\bs{X}}
\newcommand{\matY}{\bs{Y}}
\newcommand{\matZ}{\bs{Z}}

\newcommand{\bbA}{\bb{A}}
\newcommand{\bbB}{\bb{B}}
\newcommand{\bbC}{\bb{C}}
\newcommand{\bbD}{\bb{D}}
\newcommand{\bbE}{\bb{E}}
\newcommand{\bbF}{\bb{F}}
\newcommand{\bbG}{\bb{G}}
\newcommand{\bbH}{\bb{H}}
\newcommand{\bbI}{\bb{I}}
\newcommand{\bbJ}{\bb{J}}
\newcommand{\bbK}{\bb{K}}
\newcommand{\bbL}{\bb{L}}
\newcommand{\bbM}{\bb{M}}
\newcommand{\bbN}{\bb{N}}
\newcommand{\bbO}{\bb{O}}
\newcommand{\bbP}{\bb{P}}
\newcommand{\bbQ}{\bb{Q}}
\newcommand{\bbR}{\bb{R}}
\newcommand{\bbS}{\bb{S}}
\newcommand{\bbT}{\bb{T}}
\newcommand{\bbU}{\bb{U}}
\newcommand{\bbV}{\bb{V}}
\newcommand{\bbW}{\bb{W}}
\newcommand{\bbX}{\bb{X}}
\newcommand{\bbY}{\bb{Y}}
\newcommand{\bbZ}{\bb{Z}}


\newcommand{\calA}{\mcal{A}}
\newcommand{\calB}{\mcal{B}}
\newcommand{\calC}{\mcal{C}}
\newcommand{\calD}{\mcal{D}}
\newcommand{\calE}{\mcal{E}}
\newcommand{\calF}{\mcal{F}}
\newcommand{\calG}{\mcal{G}}
\newcommand{\calH}{\mcal{H}}
\newcommand{\calI}{\mcal{I}}
\newcommand{\calJ}{\mcal{J}}
\newcommand{\calK}{\mcal{K}}
\newcommand{\calL}{\mcal{L}}
\newcommand{\calM}{\mcal{M}}
\newcommand{\calN}{\mcal{N}}
\newcommand{\calO}{\mcal{O}}
\newcommand{\calP}{\mcal{P}}
\newcommand{\calQ}{\mcal{Q}}
\newcommand{\calR}{\mcal{R}}
\newcommand{\calS}{\mcal{S}}
\newcommand{\calT}{\mcal{T}}
\newcommand{\calU}{\mcal{U}}
\newcommand{\calV}{\mcal{V}}
\newcommand{\calW}{\mcal{W}}
\newcommand{\calX}{\mcal{X}}
\newcommand{\calY}{\mcal{Y}}
\newcommand{\calZ}{\mcal{Z}}




\newcommand{\veca}{\bs{a}}
\newcommand{\vecb}{\bs{b}}
\newcommand{\vecc}{\bs{c}}
\newcommand{\vecd}{\bs{d}}
\newcommand{\vece}{\bs{e}}
\newcommand{\vecf}{\bs{f}}
\newcommand{\vecg}{\bs{g}}
\newcommand{\vech}{\bs{h}}
\newcommand{\veci}{\bs{i}}
\newcommand{\vecj}{\bs{j}}
\newcommand{\veck}{\bs{k}}
\newcommand{\vecl}{\bs{l}}
\newcommand{\vecm}{\bs{m}}
\newcommand{\vecn}{\bs{n}}
\newcommand{\veco}{\bs{o}}
\newcommand{\vecp}{\bs{p}}
\newcommand{\vecq}{\bs{q}}
\newcommand{\vecr}{\bs{r}}
\newcommand{\vecs}{\bs{s}}
\newcommand{\vect}{\bs{t}}
\newcommand{\vecu}{\bs{u}}
\newcommand{\vecv}{\bs{v}}
\newcommand{\vecw}{\bs{w}}
\newcommand{\vecx}{\bs{x}}
\newcommand{\vecy}{\bs{y}}
\newcommand{\vecz}{\bs{z}}


\newcommand{\vecalpha}{\bs{\alpha}}
\newcommand{\vecbeta}{\bs{\beta}}
\newcommand{\matGamma}{\bs{\Gamma}}
\newcommand{\vecgamma}{\bs{\gamma}}
\newcommand{\matDelta}{\bs{\varDelta}}
\newcommand{\vecdelta}{\bs{\delta}}
\newcommand{\vecepsilon}{\bs{\epsilon}}
\newcommand{\matLambda}{\bs{\Lambda}}
\newcommand{\veclambda}{\bs{\lambda}}
\newcommand{\bbLambda}{\mathbbl{\Lambda}}
\newcommand{\vecmu}{\bs{\mu}}
\newcommand{\vecrho}{\bs{\rho}}
\newcommand{\matSigma}{\bs{\Sigma}}
\newcommand{\matPhi}{\bs{\Phi}}
\newcommand{\matPsi}{\bs{\Psi}}

\newcommand{\gammaOpt}{\vecgamma_{\mathsf{opt}}}
\newcommand{\GammaOpt}{\matGamma_{\mathsf{opt}}}

\newcommand{\cov}[1]{\mathsf{CN}\lc#1\rc}

\newcommand{\calCN}{\mathcal{CN}}

